Malware triage for early identification of Advanced Persistent Threat activities

In the last decade, a new class of cyber-threats has emerged. This new cybersecurity adversary is known with the name of "Advanced Persistent Threat" (APT) and is referred to different organizations that in the last years have been "in the center of the eye" due to multiple dangerous and effective attacks targeting financial and politic, news headlines, embassies, critical infrastructures, TV programs, etc. In order to early identify APT related malware, a semi-automatic approach for malware samples analysis is needed. In our previous work we introduced a "malware triage" step for a semi-automatic malware analysis architecture. This step has the duty to analyze as fast as possible new incoming samples and to immediately dispatch the ones that deserve a deeper analysis, among all the malware delivered per day in the cyber-space, the ones that really worth to be further examined by analysts. Our paper focuses on malware developed by APTs, and we build our knowledge base, used in the triage, on known APTs obtained from publicly available reports. In order to have the triage as fast as possible, we only rely on static malware features, that can be extracted with negligible delay, and use machine learning techniques for the identification. In this work we move from multiclass classification to a group of oneclass classifier, which simplify the training and allows higher modularity. The results of the proposed framework highlight high performances, reaching a precision of 100% and an accuracy over 95%

==> tex/approach.tex <==
% !TeX root = ../JISA_2018.tex
\section{The two approaches}\label{s:approach} \riccardo{sostituire completamente questa sezione e la prossima con il capitolo 5 della tesi. Il lavoro che ho fatto sulla tesi era mirato ad avere qualcosa da trasportare direttamente nell'articolo. Bisogna solo 1) tagliare approfondimenti inutili, tipo l'esempio di confusion matrix, 2) introdurre brevemente quel che è spiegato nel capitolo 4, inserendo qualche references}
Our works focus on the design of a step of a semi-automatic architecture that has to find all the malware suspected to be developed by APTs; the results of these step is than sent to human malware analysts for deeper inspection. In this section we present a brief description of our old work, based on multi-class algorithm, together with details about how we improved it using one class classifiers.
\subsection{Multi-class classifications}
In \cite{laurenza2016architecture} we develop an algorithm based on the Random Forest classifier. This algorithm first computes a \emph{confidence} average value for each class using a leave-one-out method: the confidence value is based on the distribution of element of each class in each leaf. After this computation, we derived a threshold vector composed by a threshold value for each class. The last preparatory step was to build the final model, computing the confidence of each leaf, this model is used for the prediction and the output is a confidence vector with a prediction for each class. If one or more of these scores is greater than the  threshold value of the same class, the sample will be sent in a special queue to be deeper analyzed with as label the name of the corresponding class.

\subsection{One-class classifier}
Our previous work is based on a Random Forest classifier and achieves great precision and accuracy; however, when trained over huge amount classes number, needs high level of computational resources and time for training. Moreover, each single APT sample that is going to enforce the Knowledge Base needs a total re-processing phase for Random Forest in order to reproduce each APT threshold, wasting time and resources. This weakness is the motivation of our work. Our aim is to improve APT triage concept through One-Class Classification.  Instead of relying on multi-class classification, indeed, we are going to generate, for each single APT class, an Isolation Forest, an algorithm that creates a model to identify all those elements belonging to it while discarding all \emph{anomalies}. When we want to add new samples developed by a known APT or we want to monitor a new APT, we simply do a new training phase only for this particular class. Moreover, we do not calculate any score or threshold: if a given sample passes ``unnoticed'' through each APT classifier, it is considered not related to any APT drastically reducing computational time and resources.




==> tex/experimental_evaluation.tex <==
% !TeX root = ../JISA_2018.tex
\section{Experimental Evaluation}\label{s:experiment}
To show that also this new approach can achieve good results we evaluate it with in different ways, in the first one we consider only the output of the algorithm as \emph{belong} or \emph{not belong} to any APTs, with the former that is when almost one of the classifiers predicted the sample as of its own class, the second instead is when none of the classifiers recognize the sample as a positive hit. The second kind of test instead is to verify if the algorithm is able to distinguish the correct APT developer when it found a positive result.

\subsection{Dataset}
To build the test dataset, similarly to what we have done for the previous works, we analyzed various public reports about ATPs, resulting in an updated dataset of 2196 different malware belonging to 19 groups, see table~\ref{aptclass} for details. For the test we add a set of 862 malware not developed by any APTs, to verify the correctness of our predictions.


\begin{table}[!htb]
	\label{aptclass}
	\begin{minipage}{.5\linewidth}
		\centering
		\begin{tabular}{|l|r|}
			\hline
			\textbf{Class}    & \multicolumn{1}{l|}{\textbf{Count}} \\ \hline
			Patchwork         & 559                                 \\ \hline
			APT29             & 205                                 \\ \hline
			Winnti Group      & 176                                 \\ \hline
			Carbanak          & 105                                 \\ \hline
			Volatile Cedar    & 35                                  \\ \hline
			NSA               & 13                                  \\ \hline
			Transparent Tribe & 267                                 \\ \hline
			Shiqiang          & 31                                  \\ \hline
			Roaming Tiger     & 14                                  \\ \hline
			Mirage            & 54                                  \\ \hline
		\end{tabular}
	\end{minipage}%
	\begin{minipage}{.5\linewidth}
		\centering
		\begin{tabular}{|l|r|}
			\hline
			\textbf{Class}  & \multicolumn{1}{l|}{\textbf{Count}} \\ \hline
			Lazarus Group   & 58                                  \\ \hline
			Sandwork        & 44                                  \\ \hline
			Hurricane Panda & 315                                 \\ \hline
			APT30           & 101                                 \\ \hline
			Violin Panda    & 23                                  \\ \hline
			Desert Falcon   & 45                                  \\ \hline
			Molerats        & 25                                  \\ \hline
			APT28           & 68                                  \\ \hline
			Lotus Blossom   & 48                                  \\ \hline
		\end{tabular}
	\end{minipage}
	\caption{APTs elements per classes}
\end{table}


% \begin{table}[h!] \label{aptclass}
% 	\centering
% 	\caption{APTs elements per classes.}\label{aptclass}
% 	\begin{tabular}{|l|r|}
% 		\hline
% 		\textbf{Class}    & \multicolumn{1}{l|}{\textbf{Count}} \\ \hline
% 		Patchwork         & 559                                 \\ \hline
% 		APT29             & 205                                 \\ \hline
% 		Winnti Group      & 176                                 \\ \hline
% 		Carbanak          & 105                                 \\ \hline
% 		Volatile Cedar    & 35                                  \\ \hline
% 		NSA               & 13                                  \\ \hline
% 		Transparent Tribe & 267                                 \\ \hline
% 		Shiqiang          & 31                                  \\ \hline
% 		Roaming Tiger     & 14                                  \\ \hline
% 		Mirage            & 54                                  \\ \hline
% 		Lazarus Group     & 58                                  \\ \hline
% 		Sandwork          & 44                                  \\ \hline
% 		Hurricane Panda   & 315                                 \\ \hline
% 		APT30             & 101                                 \\ \hline
% 		Violin Panda      & 23                                  \\ \hline
% 		Desert Falcon     & 45                                  \\ \hline
% 		Molerats          & 25                                  \\ \hline
% 		APT28             & 68                                  \\ \hline
% 		Lotus Blossom     & 48                                  \\ \hline
% 	\end{tabular}
% \end{table}

\subsection{Tests Details}
To show the correctness and effectiveness of our new approach, we tested it with the dataset presented before; we use a \emph{K-Cross-Folder} method for the testing, with \emph{K} equals to 10 as it is a common value in literature.\\
The test consists of use another 10-Cross-Folder test on the training set, composed of the variable set of nine folders, in order to find the best parameters for each classifier; in particular we take all the malware developed by APTs, divide them in ten folders and than, changing each time the \emph{Test folder}, we obtaine the couples of training and test set. Then we applied another foldering on only the training set, using the variable test as a validation for finding the best arguments; as explained in \ref{parameters} we decided to focus on precision and accuracy for achieve a better triage phase.\\
At the end of this step, we use the entire training set, made by the nine initial folder, as the input for the creation of the One Class Classifiers, using the parameters selected before.\\
The last step of the tests is to use the classifiers on each test folder composed by malware developed by APTs, adding also the set of malware that are not part of these threats. In this way we can check both if our algorithm can correctly identify if a malware belong to an APT and also which APT developed it.\\
As explained at the beginning of the section, we present the results using two different methods, first we show how our algorithm is good into \emph{APT detection}, in practice we show that our solution can correctly find malware that are developed by one of the monitored APTs and thus raise an alert for deep analysis. The second method is to show that in addition to detect this class of malware, our work can suggest with high accuracy to which APT the malware belongs.

\subsection{Test Results}
In table \ref{detection} we show the Confusion Matrix of the first test: it is clear that our system achieves a total of 0 false positive, thus we do not label as developed by APTs any malware that is not related to these kind of threats. In this way it is possible to save the limited resources needed for a deeper analysis like human analysts. \\
Of course, we are interested in detect advanced attacks, so we have to find an high number of malware developed by these adversaries: our system is capable of correctly identify more than 1700 of them, failing only for less than 500 cases. As explained before, these malware that are not recognized by any Classifier will not be excluded by further analysis of the security expert: simply they are not prioritized to a prompt and deep analysis.\\
\begin{table}[]
	\centering

	\label{detection}
	\begin{tabular}{ll|r|r|}
		\cline{3-4}
		                                                     &                                    & \multicolumn{2}{c|}{\textit{Predicted}}                                      \\ \cline{3-4}
		                                                     &                                    & \multicolumn{1}{l|}{\textbf{non-APTs}}  & \multicolumn{1}{l|}{\textbf{APTs}} \\ \hline
		\multicolumn{1}{|c|}{\multirow{2}{*}{\textit{True}}} & \textbf{non-APTs}                  & 8620                                    & 0                                  \\ \cline{2-4}
		\multicolumn{1}{|c|}{}                               & \multicolumn{1}{c|}{\textbf{APTs}} & 495                                     & 1711                               \\ \hline
	\end{tabular}
	\caption{APTs Detection confusion matrix}
\end{table}

Table \ref{detection_measures} shows, instead, the results in term of quality measures: we can achieved our goal of maximize the precision, in fact we obtain a 100\%, maintaining even an accuracy of 95\%. Our system can't achieve a very high recall, but this was an expected result and it is not a real problem, due to the fact that this is only a preliminary phase of a complex architecture and it has only the goal of detecting most \emph{dangerous} malware as possible.\\

\begin{table}[]
	\centering
	\label{detection_measures}
	\begin{tabular}{|c|c|c|c|}
		\hline
		\textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} \\ \hline
		95\%              & 100\%              & 77\%            & 87\%        \\ \hline
	\end{tabular}
	\caption{APTs Detection quality measures}
\end{table}

However our system is designed for a more specific objective: to identify which APT group is the author of these advanced malware. Table \ref{identification} highlights the identification results: in this table we consider only malware that are labeled as belonging to APTs, hence we now analyze the performance of each classifier in the identification process of its relative samples, over all samples that in the triage phase have been detected as developed by APTs. Our system can correctly label more than 1600 malware from a dataset of about 2000, thus we can give useful additional information for the following deeper analysis. Moreover, a wrongly assigned label is not a great failure, due to the fact that these malware still deserve a richer inspection, since they are developed by APTs.\\
\begin{table}[]
	\centering
	\label{identification}
	\begin{tabular}{lc|c|c|}
		\cline{3-4}
		                                                     & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{\textit{Predicted}}                        \\ \cline{3-4}
		                                                     &                       & \textbf{Other APTs}                     & \textbf{Correct APT} \\ \hline
		\multicolumn{1}{|c|}{\multirow{2}{*}{\textit{True}}} & \textbf{Other APTs}   & 41475                                   & 249                  \\ \cline{2-4}
		\multicolumn{1}{|c|}{}                               & \textbf{Correct APT}  & 533                                     & 1663                 \\ \hline
	\end{tabular}
	\caption{APTs Identification confusion matrix}
\end{table}
In term of quality measures, table \ref{identification_measures} shows that our system obtain a very high accuracy (98\%), thus confirming the correctness of our solution. Even if the other measures aren't so high, we have to consider that they are expressed in relation to the rightness of the label, but that in terms of overall APTs Detection, these measures are much higher.\\
\begin{table}[],
	\centering
	\label{identification_measures}
	\begin{tabular}{|c|c|c|c|}
		\hline
		\textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} \\ \hline
		98\%              & 86\%               & 75\%            & 80\%        \\ \hline
    \end{tabular}
    \caption{APTs Identification quality measures}
\end{table}

==> tex/methodology_laurenza.tex <==
% !TeX root = ../JISA_2018.tex
\section{Methodology in details}\label{s:methodology}
\giuseppe{Va bene qui o meglio includerlo in altra sezione?}
In this section we will provide details about the triage process, some of them are similars to what we did in the previous article, but we prefer to report also here to allow a better understanding of the entire phase.

\subsection{Feature Extraction}
Our triage step starting from the features extraction; as explained in the other parts of the paper, we need to evaluate samples as fastest as possible, so we decide to use only static analysis tools. For this work we used two famous open-source static analysis tools: PEframe\footnote{https://github.com/guelfoweb/peframe} and Vivisect\footnote{https://github.com/vivisect/vivisect}; the former can obtain many information from the analysis of the headers of an executable file, instead the latter is a complex framework that we used mainly to extract metadata about the functions, included the ones \emph{hidden} in not executable areas.  We can roughly divide these features in seven classes, table \ref{t:features} shows details about the composition of the features set.
\begin{table}[] \label{t:features}
	\centering
	\caption{Features classes.}\label{table1}
	\begin{tabular}{|l|r|}
		\hline
		\textbf{Class}               & \multicolumn{1}{l|}{\textbf{Count}} \\ \hline
		Optional Header              & 30                                  \\ \hline
		MS-DOS Header                & 17                                  \\ \hline
		File Header                  & 7                                   \\ \hline
		Obfuscated String Statistics & 3                                   \\ \hline
		Imports                      & 158                                 \\ \hline
		Function lengths             & 50                                  \\ \hline
		Directories                  & 65                                  \\ \hline
	\end{tabular}
\end{table}

\subsection{Features Reduction}
Due to the high number of features, we decide to apply \emph{Linear Discriminant Analysis} in order to reduce the dimensionality of features set. We choose LDA because of its simplicity and we map the features in a number of projection equals to the number of classes.
\giuseppe{sinceramente qui non sapevo che scrivere, al massimo pensavo di aggiungere una breve spiegazione di cosa è LDA}

\subsection{Parameters Details}
\label{parameters}
The implementation of Isolation Forest algorithm that we used in our approach allows the management of only two parameters: \emph{contamination} and \emph{number of estimator}; the former refers the tolerance value of the classifier during the model creation, the second instead is the number of trees the algorithm has to use. According to the requirements of a \emph{Triage algorithm} we decided, as we did also in the previous work, to maximize the precision score and the accuracy score. we took this decision because human analysts are a very limited resource and thus we must be sure to give to them only sample that deserve to be manual analyzed, even if in this way we fail to recognize some malware developed by APTs. Thanks to the fact that the analysis is composed of many different step, we can add other slower steps after the triage one, likely one similar algorithm based on dynamic features, thus the malware that are not find during the triage phase can be identified in the next part of the architecture.

\subsection{Training Phase}
To make possible the analysis of new malware, we should preventively build the One Class classifiers, one for each APT. The first thing is to find the better parameters, an advantage of this algorithm is that we can build a model for each class, so we can tune individually tune them. To do this we simply test our classifiers with the training set, using a 10 folder validation approach and a wide range of arguments in different combination. The output of the tuning is a number of classifiers each of the number of the classes. After the tuning, we train our models with the full training set and produce the final classifiers.

\subsection{Triage Phase}
After a new sample arrives in the architecture, it will be first analyzed by different static and analysis tools; after the static analysis step is concluded, our feature extractor built the features vector for the identification. The next step is the analysis trough the previous trained One Class Classifiers, if almost one of them produces a positive label, an alert is raised and different measures can be taken, like send it to a team of human analysts or use some \emph{expensive} deep analysis tool that is used only for special cases. 
